Protection or punishment? relating the design space of parental control apps and perceptions about them to support parenting for online safety

Parental control apps, which are mobile apps that allow parents to monitor and restrict their children's activities online, are becoming increasingly adopted by parents as a means of safeguarding their children's online safety. However, it is not clear whether these apps are always beneficial or effective in what they aim to do; for instance, the overuse of restriction and surveillance has been found to undermine parent-child relationship and children's sense of autonomy. In this work, we investigate this gap, asking specifically: how might children's and parents' perceptions be related to how parental control features were designed? To investigate this question, we conducted an analysis of 58 top Android parental control apps designed for the purpose of promoting children's online safety, finding three major axes of variation in how key restriction and monitoring features were realised: granularity, feedback/transparency, and parent-child communications support. To relate these axes to perceived benefits and problems, we then analysed 3264 app reviews to identify references to aspects of the each of the axes above, to understand children's and parents' views of how such dimensions related to their experiences with these apps. Our findings led towards 1) an understanding of how parental control apps realise their functionalities differently along three axes of variation, 2) an analysis of exactly the ways that such variation influences children's and parents' perceptions, respectively of the usefulness or effectiveness of these apps, and finally 3) an identification of design recommendations and opportunities for future apps by contextualising our findings within existing digital parenting theories.

==> 4.ResultsReviewsA.tex <==
%==========================================
%==========================================
%=================archive==================
%==========================================
%==========================================

\subsection{Thematic Analysis of Reviews}

This section presents an overview of the primary themes pertaining to
the reasons children and parents, respectively, liked or disliked
features provided by parental control apps.

% \textcolor{red}{I can see why the map between features and reviews is important, at least a broad indication about the level of feature granularity these review discussions are above?}

\subsubsection{Children's viewpoints:}
We first start with children's perspectives; the children expressed a 
variety of views on what they hated about parenting apps, which we 
believe offers a rich starting point for understanding the potential
harms and limitations of these apps.

\vspace{1em}

\noindent\textbf{Disliked being overly surveilled and restricted} - 
The most common grievance was the view that these apps not only
enabled but encouraged parents to set up overly restrictive controls
and excessive surveillance.  Kids expressed resentment at the
extent of both the restrictions and their surveillance, and
reflected on the effects lives, welfare, and activities:

\begin{small}
\begin{quote}
  This literally blocks everything, I can't even read e-books on my
  phone. 
\end{quote}
\end{small}

\begin{small}
\begin{quote}
  This is insane. Now they can see EVERYTHING! From my browsing history
to what apps I downloaded, even my texts! Worst app ever! 
\end{quote}
\end{small}

\noindent Kids reflected on a variety of secondary effects of excessive
restrictions and surveillance.  One child discussed that they felt
that, beyond violating their privacy, it was particularly wrong that
their parents' access to their messages would compromise their
friends' privacy as well:

\begin{small}
\begin{quote}
  they can eves drop on your convos and stuff that you dont want them
  to hear [...] not only is it a violation of my
  privacy that i didnt permit, but it is of friends too that parents
  dont know about
\end{quote}
\end{small}


\noindent The pervasiveness and constancy of surveillance made it feel to one
as if these apps enabled their parents to ``stalk'' them:

\begin{small}
\begin{quote}
    I hate this app my mom is like stalking my life!!
\end{quote}
\end{small}

\noindent Even when not restricted, the perception that their social communications were
being surveilled by their parents had a chilling effect that  indirectly 
forced them to cease communicating and be cut off from their friends.

\begin{small}
\begin{quote}
  I can't talk with my friends anymore, everything will be recorded! 
\end{quote}
\end{small}

\noindent Several comments discussed longer-term effects such restrictions were having on their well-being. One view was that restrictions were directly and immediately harmful because they broke essential lines of social support.

\begin{small}
\begin{quote}
  This is stupid. absolutely awful. this will ruin people's lives. I
  had severe depression and the only thing keeping me from killing my
  self was my friend who I could only talk to online. Now I'm fine but
  if I lose contact with that friend I will most likely get my
  depression back. Horrible and stupid app. 
\end{quote}
\end{small}

% \noindent Time-based restrictions were seen to disrupt children's social lives as well
% because it prevented them from communicating when plans were being made.

% \begin{quote}
% I'm in year 9 and all my friends are always making plans at the night time but I can only see these messages at 7 in the morning by that time, everything has been planed who's going and what time soon they forget about me I'm now excluded and lonely just because of an app on my phone do not use this for your children please it's not the right thing to do.(K)
% \end{quote}

\noindent Beyond cutting off lines of social support, restrictions were seen to
prevent kids from apps and activities that they normally used to cope
with boredom and isolation, further undermining well-being:

% \begin{quote}
%  I can't play a lot of games, and I can't watch YouTube. The only
%  friends I have isn't in town lives 15 miles away and my parents
%  never want to drive me there so I've sat in my room for weeks doing
%  nothing and practically getting depressed because there is
%  literally NOTHING I can do! 
% \end{quote}
\begin{small}
\begin{quote}
 I can't play a lot of games, and I can't watch YouTube. I've sat in my room for weeks doing
 nothing and practically getting depressed because there is literally NOTHING I can do! 
\end{quote}
\end{small}

% \noindent The consequences extended from the digital to the real world; 
% one discussed how being cut-off from communications channels led them to
% be excluded from real-world social opportunities, further exacerbating
% isolation, feelings of being cut-off, and loneliness.

% \begin{quote}
%   I'm in year 9 and all my friends are always making plans at the
%   night time but I can only see these messages at 7 in the morning by
%   that time everything has been planed who's going and what time soon
%   they forget about me I'm now excluded and lonely just because of an
%   app on my phone do not use this for your children, please it's not
%   the right thing to do.
% \end{quote}

\noindent Beyond the social and emotional aspects of children's' lives, a few comments 
connected these restrictions to developmental and educational harms-namely,
how such restrictions impeded learning by depriving them of experiences 
and learning opportunities:

\begin{small}
\begin{quote}
  The internet is where kids discover and learn new things. And by
  restricting it, you're denying them that ability.
\end{quote}
\end{small}

% \noindent Another child commented that restrictions were pointless, and learning
% about safety was both necessary and inevitable anyway due to their
% ineffectiveness:

% \begin{small}
% \begin{quote}
%   My parents also used other filters, all of which I could disable in
%   at least 2 different ways. I guess my point is... maybe kids can
%   learn for themselves what's safe and what isn't. They are going to
%   get uncensored access sooner or later. 
% \end{quote}
% \end{small}

\noindent\textbf{Role of Parenting Apps: Unnecessary, Punishment, or Lazy Parenting} - A second theme related to the roles parenting apps were meant to play.  Several of the children's comments expressed confusion or questioned the role these apps were supposed to play in keeping them safe. One view that these apps were  fundamentally redundant because they were already old enough or  competent enough and to be able to keep themselves safe:

%  \begin{quote}
%   I get why you use it on younger kids but I am 13 already, I deserve
%   to have control over my own life! (K)
%  \end{quote}

\begin{small}
 \begin{quote}
   I'm a 4.0 student.  Who is able to manage her school work and
   screen time by herself thank you very much. I'm old enough to know
   what's good and bad, but my mom just doesn't understand that. 
 \end{quote}
\end{small}

\noindent Other kids lamented that these apps were unnecessary because kids could be told what to do, and trusted to keep what they were told. In a sense, the use of apps to force represented a failure of trust.
 
\begin{small}
 \begin{quote}
    How bout you try and talk to them about your phone usage first, see if they'll make a change for you first, then go from there. Think twice before you destroy you kid's trust like this. I understand there's kids who need to get their head straight. But for those like me who are focused in school and a well-rounded kid, I feel all you need to do is talk to them.
 \end{quote}
\end{small}

%about their phone usage. I certainly would have made a change in my life to limit my phone usage, but I wasn't given a warning.. I was quickly bombarded with all these restrictions. 

\noindent The perception that parents are not trusting them made children question the point of these apps. In some cases, children regarded the use of these apps as purely for punishment.
%  \begin{quote}
%     My mom overreacted and got this app, they have complete control over your phone ounce they get this app. If you are a parent that wants this app I would reconsider getting this and punish your child a different way. Kids will feel punished not only that but, it actually has a affect on how we think. Instead of us being punished, parents should be blamed for dictating their children to use this app. (K)
%  \end{quote}

\begin{small}
  \begin{quote}
    If you are a parent that wants this app I would reconsider getting this and punish your child a different way. Instead of us being punished, parents should be blamed for dictating their children to use this app.
 \end{quote}
\end{small}
 
\noindent Some children continued the criticise the bad parenting styles that these apps nudged their parents into. Apart from parents being overly-protective (as we previously reported), children also accused parents of being lazy and using the apps as substitutes for parenting. 
\begin{small}
 \begin{quote}
      Yes, it's good to be one step ahead, but having an app to do it for you? You might as well call child protective services if you're that lazy. 
 \end{quote}
\end{small}

\noindent\textbf{Perceived benefits: Keeping them safe and productive} - 
When children understand why the apps are for, they reported more positively about the apps. Several of the comments by children pointed out that the apps helped to keep them safe online from inappropriate things:
\begin{small}
 \begin{quote}
     I know this may sound crazy from the kids view,  but I love this now! It fits me and my phone perfectly, and my mom knows that I am safe on my phone without having to go to any other horrible apps.
 \end{quote}
\end{small}

\noindent Other children who suffered from addiction online appreciated how the apps dragged them out of that cycle:
\begin{small}
\begin{quote}
     This is AWESOME! I'm a kid so I got this app in order to keep myself in check on my screen time because I am an internet addict. I'm so much happier now! It makes it absolutely impossible to get around!
 \end{quote}
\end{small}

\noindent Beyond the positive impacts online, children also appreciated how the apps help with their time offline. Some children commented that they are now able to become more productive and spend more time with their families:
%  \begin{quote}
%      Although i am only 11,I really find this app useful and informative. I really love this app since I want to be more productive and use my time for more crucial tasks. (K)
%  \end{quote}
\begin{small}
 \begin{quote}
     When my mom and dad put this on my phone and tablet at first I hated it. but then I realised with a limited amount of time I spent more time with my family and do actual work. I hope this inspires you to limit yourself with the amount of time you spend staring at useless junk. 
 \end{quote}
\end{small}

% 
\subsubsection{Parents' views and counterpoints}
In this section, we report a subset of themes of parents' reviews that correspond to major themes, and those that represent counterpoints to the children's themes above.

\noindent\textbf{Peace of mind, protection not punishment} - Parents were generally positive about the apps, generally seeing parental control apps as effective at helping them support their primary goal, which was to keep their children safe.  These parents felt such apps gave them ``peace of mind'':

% \begin{quote}
% 	I love this app. I have a 10 year old son that I just recently found out was doing inappropriate things on the Internet with his phone, like viewing porn on YouTube , needless to say I was highly upset , but with this app I Have some peace of mind. I have full control of what he downloads and views on the net , in addition. I can limit how much time he can spend on his phone, all form [sic] my device. I also downloaded kids YouTube, which keeps him from viewing adult content. I highly recommend this app.
% \end{quote}
\begin{small}
\begin{quote}
	I love this app. I have a 10 year old son that I just recently found out was doing inappropriate things on the Internet with his phone, like viewing porn [...] but with this app I Have some peace of mind. I have full control of what he downloads and views [...] all form [sic] my device. 
\end{quote}
\end{small}

\noindent With regard to children feeling punished, some parents showed awareness of this perception and provided advice to others about how to avoid it. One advocated for discussing the purpose of the tool with the child to frame it within an educational and protective context:

\begin{small}
\begin{quote}
	Talk with them about the reason you’re doing this. Allow your kids to help you set limits and rules. Show them you trust them. Emphasize it as a tool for them to stay safe and to learn important skills, rather than simply a way to punish them.
\end{quote}
\end{small}

\noindent Other parents struggled to communicate this, expressing that their children indeed felt punished:

\begin{small}
\begin{quote}
	I want to make sure no more creeps are following her. I took away all of her access to her electronics and she felt like she was being punished! She didn’t do anything wrong, so she shouldn’t have to feel that way! Hopefully, one day she will see the bigger picture...
\end{quote}
\end{small}

\noindent\textbf{Supports, rather than enacts parenting}- One parent felt it was necessary to remind other parents to see such apps merely as one of an arsenal of tools to retain an active involvement in parenting:

\begin{small}
\begin{quote}
	This is a great tool. Easy to use. Straightforward. Just enough options. I use this tool to help, but in noway does it replace being a good parent watching over their child. It should not be the only arrow in your quiver, and you should not expect it to do your parenting for you.
\end{quote}
\end{small}

\noindent \textbf{Diverse attitudes: Privilege not a right} - Parents expressed multiple opposing views around children's rights to privacy. Several expressed sympathy, saying they exercised caution and tried to be respectful in the use of restrictions and monitoring features, negotiating rules in advance:

\begin{small}
\begin{quote}
	This app is perfect. We do homeschooling, and we know it’s important to let our kids stay connected with their friends. We adjusted the setting so that our kids can still chat online during scheduled study times...”
\end{quote}
\end{small}
\begin{small}
\begin{quote}
	For best results, track your kids' usage for a while before limiting anything, and when restricting usage, have the discussion about what’s reasonable so you can come to an agreement. Resist the temptation to go \emph{full fascist} right away even though you are probably extremely frustrated when you finally download this app.
\end{quote}
\end{small}

% \noindent Some parents continued to add on to the argument by stating that children forced under restrictions mean they don’t get an understanding of the importance or significance of the restrictions or risks online:
% \begin{small}
% \begin{quote}
% 	A child who grew up with no limitations placed but with the knowledge that limitations and time management are important will place limitations on themselves and manage their time. A kid who is forced with these limitations may not know the importance of limitations on time doing other things that aren’t their responsibilities/obligations. This kid will grow up thinking limitations are stupid and probably not place limitations on themselves when they are alone in the real world. 
% \end{quote}
% \end{small}

\noindent An opposing view was expressed by some parents who questioned whether children deserved any rights to privacy at all. One stated that since parents were paying for the phone, they should be able to set the rules:
\begin{small}
\begin{quote}
	Don’t listen to these spoiled children. I pay the bills. I control the phone. You want to control you pay the bills! Very very simple equation! It’s a shame how kids here actually can fathom the thought of ``rights'' while living in their parents' home. Who made that joke up?
\end{quote}
\end{small}

\noindent In some cases, parents also talked about how their duty as parents to keep kids safe outweighed any claim to rights:
\begin{small}
\begin{quote}
	When it comes to social media, kids don't need privacy. It’s not even about the child as much as it is about others preying on them. I would hope none of the negative reviews are from parents. You should monitor everything your children do. That is our job as parents.
\end{quote}
\end{small}

\noindent A more lenient version of this was the view that rights to autonomy/privacy should be an earned privilege, not a fundamental right:
\begin{small}
\begin{quote}
	If you want more trust privacy, prove you can handle it with good choices to show your parents you are trustworthy!
\end{quote}
\end{small}

\noindent Others viewed their children as being too young to make decisions for themselves until they become adults, regardless of their age:
\begin{small}
\begin{quote}
	It’s not that we don’t trust them, but studies show they can’t make decisions or assess risk like adults can until age 25 or so.
\end{quote}
\end{small}

\noindent\textbf{Other concerns: privacy and disclosure to third parties}- Similarly, a few children reflected on how much access to private data apps had, and that their use represented a fundamental violation of
what they were taught about being cautious with apps accessing
personal info at school:
\begin{small}
\begin{quote}
    My school kept telling us to protect our personal information online, but what parents did here directly contradicts what I was told. (K)
\end{quote}
\end{small}

\noindent Parents similarly expressed privacy concerns relating to the potential 
for developers of parenting apps to collect and abuse information 
about their children's' behaviour sensed and collected through the app:
\begin{small}
\begin{quote}
    Forget the children's privacy for a moment. How much DATA MINING is this company doing?? They are not only getting all your information from FB, but they also learn everything about your child\'s behavior. This app isn't meant for the parents. It's meant for the company to harvest data.
\end{quote}
\end{small}

\noindent Parents also criticised how heavy surveillance on children would train them into the mindset of getting used to, thus not caring about personal information as they grow up:
\begin{small}
\begin{quote}
    Considering how little privacy we have left, I fell this app is training kids to feel ok with the fact their data is being spread all over the internet by advertisers and making it normal to feel like there is no privacy. (P)
\end{quote}
\end{small}





==> 4.ResultsReviewsB.tex <==
%==========================================
%==========================================
%=================archive==================
%==========================================
%==========================================
\subsection{How do features relate to perceptions?}

\begin{figure}[h!]
\caption{\emph{Mapping feature analysis to perceptions-} Here we connect all the variations of app features along each of the 3 axes against reviews about them, and indicate whether children and parents primarily viewed such features \emph{positively}, \emph{negatively} or \emph{conflicted}, or expressed no view (x). \label{fig:mapping}}
\label{fig:compare}
\centering
\includegraphics[width=1\textwidth]{mapping.png}
\end{figure}

Thus far, we have analysed apps and how features varied along three axes in Section 4.1, and, separately, thematically coded perceptions of parenting apps by both parents and children in Section 4.2.  In this section, we aim to understand how particular aspects of how features are realised (along the axes of variation), and how that maps to parents and children's perceptions. We use a grounded approach to code our reviews. However, interesting matching between our previous feature analysis and users' perceptions (reviews) can be identified (see \textbf{Figure \ref{fig:mapping}}).

\subsubsection{Granularity}
\begin{itemize}
    \item Both parents and children disliked the coarsest level of granularity, \emph{all-or-nothing}, corresponding to over 30\% of apps (\scalebox{0.5}{ALL-OR-NOTHING}32\%)
    \item Both parents and children liked apps providing an \emph{intermediate level of granularity}, which usually consisted policies based on meaningful/convenient sets, which were approximately as common as the previous category \\(\scalebox{0.5}{CONTROL-CATEGORY-AGE}32\%, \scalebox{0.5}{MONITOR-CATEGORY}18\%, \scalebox{0.5}{MONITOR-SUSPICIOUS}16\%)
    \item Children disliked apps providing highly granular controls, while some parents strongly liked these. Such designs are prominent in apps( \scalebox{0.5}{CONTROL-PER-APP}34\%, \scalebox{0.5}{MONITOR-EXPLICIT-INFO}40\%):
\end{itemize}

Both parents and children disliked when apps only offered control in an all-or-nothing fashion. They criticised such apps as unreasonable, inconvenient and annoying. On the other hand, most children didn't like apps providing the most granular affordances, especially in terms of monitoring, which enabled their parents to see very detailed information. Interestingly, parents held conflicted opinions; while some expressed sympathy and reported that they didn't want to know ``everything'', others cherished being able to know every single detail of their children's lives.  In terms of restriction, whilst some parents loved being able to adjust the setting on a per-app/website basis, others complained about the effort and knowledge required from them to do that.

Most parents and children liked intermediate levels of granularity, which consisted of apps supporting controls grouped into meaningful categories, such as app genres and categories, age-appropriateness, and support for filtering monitored data for only `suspicious content'. This was seen not only as convenient for parents, but also seen to support setting of  boundaries in a more flexible manner. Similarly, both parents and children appreciated how some apps enabled different children, especially older ones, with different level of freedom: 
% \begin{quote}
%     This is an amazing app that even my daughter can appreciate! She has type 1 diabetes and uses her tablet to keep track of her blood glucose levels. While she loves playing games, watching videos and TV, her mood and attention span suffer if she spends too much time staring at screens (she even notices, although she still moans when we remind her of her 2 hours a day TV/gaming/tablet limit). With this app and its companion, I can lock down all apps that count towards her daily screen limit but leave open her diabetes app and a few educational apps.  (P)
% \end{quote}
\begin{small}
\begin{quote}
    This is just great. It allows age-appropriate control, so giving us more freedom as we get older. (K)
\end{quote}
\end{small}

\subsubsection{Feedback/Transparency}
\begin{itemize}
    \item Both parents and children dislike features that support little feedback/transparency. However, such features are prominent (\scalebox{0.5}{RULES-NO-SHOW}14\%, \scalebox{0.5}{MONITOR-NO-SHOW}32\%, \scalebox{0.5}{ONLY-RULES-AT-MOMENT}20\%)
    \item Both parents and children agreed features should support feedback/transparency. However, only 20\% apps offer these  (\scalebox{0.5}{RULES-PAGE}12\%, \scalebox{0.5}{MONITOR-PAGE}8\%)
    \item Both parents and children like features that have high feedback/transparency. However, such features are largely scarce (\scalebox{0.5}{RULES-EXPLAIN}6\%, \scalebox{0.5}{MONITOR-SELF-TRACK}14\%, \scalebox{0.5}{SHOW-KIDS-INFO}4\%) 
\end{itemize}

Both children and parents expressed their dislike of feature designs that supported no feedback/transparency, which were sadly the most common feature designs. In terms of screen rules, they complained about how some app doesn't let children know what their screen rules are when such system is missing, children found themselves in the position of had to work things out based on trial-and-error. In terms of monitoring, children felt insecure when not knowing what their parents can see about them. Rules without prior acknowledgment were sometimes presumed to be annoying by children. For example, both parents and children brought up that prior warnings on time remaining are important. Otherwise, children will feel upset due to the sudden cut-off.

Both parents and children liked feature designs that supported children's understanding of their online boundaries. In terms of restriction, both parents and children brought up how they like apps offering children with clear screen rule pages so their children will be better informed instead of suffering from being turned down at the moment when they are trying to do some online activities. In particular, Many kids pointed out how they like being offered with explanations on why a website/app is blocked, which made them feel less confused and more respected as a consequence:
\begin{small}
\begin{quote}
    Not the best but definitely better than the previous one. Now I know why the websites are blocked. They give you explanations and things like that. I mean, I disagree with them all the time, but at least they tried to show some respect! (K)
\end{quote}
\end{small}

Some apps also showed children with their detailed online activities (rather than just a page on the list of things that will be monitored). Through this process, children were also acknowledged of their digital use online. Both parents and children reported this as helping to raise children's awareness of their time online, thus helped them make more informed decisions on their time:
\begin{small}
\begin{quote}
    It is just a simple way to track your phone usage. It has helped me be more aware of how much I spend on my phone, and I do spend too much time on games sometimes. It has helped me lessen that amount. I love this app! (K)
\end{quote}
\end{small}


\subsubsection{Communications Support}
\begin{itemize}
    \item Both parents and children disliked apps that failed to support any communication. While nearly 70\% of apps fall into this category (\scalebox{0.5}{DONT-KNOW-EXIST}14\%, \scalebox{0.5}{NO-MEANS}54\%)
    \item Both parents and children liked features that support some communication. While only around 30\% of apps support that  (\scalebox{0.5}{SEND-MESSAGE}18\%, \scalebox{0.5}{REWARD}12\%, \scalebox{0.5}{BOTH-DEVICE}2\%)
    \item Parents in particular, loved features that support active parenting. However, limited apps offer these features  (\scalebox{0.5}{CO-CONFIG}4\%, \scalebox{0.5}{PARENTING-TIPS}10\%)
    
\end{itemize}

Most apps offered no means for negotiating screen rules (54\%), which is disfavoured by both parents and children.  They complained about how inconvenient it was, especially when parents could not physically adjust settings in person.

In general, parents and children liked designs that supported any form of communication. Whether it's a negotiation on screen time through a reward system, or simply having a send message function to alter the settings. Children, in particular, loved the co-configuration designs that allowed them to sit down with their parents and reach mutual agreement on their boundaries. Meanwhile, parents also reported their favour towards feature designs that supported or coached them on conversations with their children. And they found designs like parenting tips particularly useful. For feature designs in this group, parents and children hole quite similar opinions. They either both loved it, or both hated it. Interestingly though, the reason they liked the reward systems was quite different.  While children talked about how they love the fun or getting used to the reward systems, parents tend to think that their children learned important internal values throughout the process, such as self-discipline or being responsible:

\begin{small}
\begin{quote}
    I am a kid, and I think it's awesome because your parents can block you at certain times, and you can do things to earn more time.;-) It's super fun! P.S. Kids, if u don’t like it, u must be messed in the head! It's such a great app!!!;- (K)
\end{quote}
\end{small}

\begin{small}
\begin{quote}
    They WANT to do their chores to earn more screen time :) It is teaching them time management, and they are more responsible with their tablet use now. (P)
\end{quote}
\end{small}

\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.5\textwidth]{practices.png}
  \end{center}
    \caption{\textit{Most and Least Favoured Design Practices} - Here we plot the apps under three axes of variations, the level of granularity is represented by different shades of colour\label{fig:practices}}
\end{wrapfigure}



\subsubsection{Most and Least favoured combinations by Parents and Children}
\hfill \break
Mapping our feature analysis with review analysis, we concluded the most and least favoured combinations of feature designs (see \textbf{Figure \ref{fig:practices}}):

\begin{itemize}
    \item Least Favoured, were the apps with feature designs low on all three dimensions: low granularity, low feedback/transparency, and low communications support.
    \item Most Favoured were the apps with feature designs high on both feedback/transparency and communications support, while offering a medium level of granularity.
\end{itemize}

% Interestingly, our results echo with the actual app ratings. The average rate for the apps in the least favoured box was 2.5, while the one in the most favoured box being 3.7.

% \begin{figure}[tp]
% \caption{Most and Least Favoured Design Practices\label{fig:practices}}
% \centering
% \includegraphics[width=0.6\textwidth]{practices.png}
% \end{figure}



